The Academic Midas Touch: An Indicator of Academic Excellence

The recognition of academic excellence is fundamental to the scientific and academic endeavor. However, the term "academic excellence" is often interpreted in different ways, typically, using popular scientometrics such as the H-index, i10-index, and citation counts. In this work, we study an under-explored aspect of academic excellence -- researchers' propensity to produce highly cited publications. We formulate this novel perspective using a simple yet effective indicator termed the "Academic Midas Touch" (AMT). We empirically show that this perspective does not fully align with popular scientometrics and favorably compares to them in distinguishing award-winning scientists.

==> highlights.tex <==
Introducing "Academic Midas Touch" (AMT) for evaluating academic excellence.
AMT validated as a valuable tool for academic excellence in mathematicians.
Academic excellence recognition is vital in academia and uses computational methods.

